Improving tobacco social contagion models using agent-based simulations on networks

Over the years, population-level tobacco control policies have considerably reduced smoking prevalence worldwide. However, the rate of decline of smoking prevalence is slowing down. Therefore, there is a need for models that capture the full complexity of the smoking epidemic. These models can then be used as test-beds to develop new policies to limit the spread of smoking. Current models of smoking dynamics mainly use ordinary differential equation (ODE) models, where studying the effect of an individual's contact network is challenging. They also do not consider all the interactions between individuals that can lead to changes in smoking behaviour, implying that they do not consider valuable information on the spread of smoking behaviour. In this context, we develop an agent-based model (ABM), calibrate and then validate it on historical trends observed in the US and UK. Our ABM considers spontaneous terms, interactions between agents, and the agent's contact network. To explore the effect of the underlying network on smoking dynamics, we test the ABM on six different networks, both synthetic and real-world. In addition, we also compare the ABM with an ODE model. Our results suggest that the dynamics from the ODE model are similar to the ABM only when the network structure is fully connected (FC). The FC network performs poorly in replicating the empirical trends in the data, while the real-world network best replicates it amongst the six networks. Further, when information on the real-world network is unavailable, our ABM on Lancichinetti-Fortunato-Radicchi benchmark networks (or networks with a similar average degree as the real-world network) can be used to model smoking behaviour. These results suggest that networks are essential for modelling smoking behaviour and that our ABM can be used to develop network-based intervention strategies and policies for tobacco control.

==> extra.tex <==

\subsection{Contributions and structure of paper}

 We identify three major contributions of the model.
 
 First, we show that the smoking dynamics change drastically based on the underlying network topology of the population. Besides comparing the ABM on different networks, we also compare it with the equivalent compartmental model and show that the population dynamics of the ABM on a fully connected network is equivalent to the traditional compartmental model qualitatively.
 
 Second, we identify individuals and groups of individuals to target, who can potentially act as influencers to maximise smoking cessation. We do this by studying the position of each agent on the network and its network properties.
 
 Finally, we show that quitters are more efficient at convincing smokers to quit as compared to susceptible population.

 The paper is organised as follows: In Methods, we introduce the base compartmental model used to develop the ABM along with the choice of parameters, and then discusses the general framework for the ABM. In the Results section, we elaborate the results for the ABM for the following network topology: Fully Connected network, BA network, ER network. Based in the network analysis of the population, we further discuss the policies best suited for each kind of network studied. 
 
 
 
 
 
 
 
 % Place tables after the first paragraph in which they are cited.
\begin{table}[!ht]
\begin{adjustwidth}{-2.25in}{0in} % Comment out/remove adjustwidth environment if table fits in text column.
\centering
\caption{
{\bf Table caption Nulla mi mi, venenatis sed ipsum varius, volutpat euismod diam.}}
\begin{tabular}{|l+l|l|l|l|l|l|l|}
\hline
\multicolumn{4}{|l|}{\bf Heading1} & \multicolumn{4}{|l|}{\bf Heading2}\\ \thickhline
$cell1 row1$ & cell2 row 1 & cell3 row 1 & cell4 row 1 & cell5 row 1 & cell6 row 1 & cell7 row 1 & cell8 row 1\\ \hline
$cell1 row2$ & cell2 row 2 & cell3 row 2 & cell4 row 2 & cell5 row 2 & cell6 row 2 & cell7 row 2 & cell8 row 2\\ \hline
$cell1 row3$ & cell2 row 3 & cell3 row 3 & cell4 row 3 & cell5 row 3 & cell6 row 3 & cell7 row 3 & cell8 row 3\\ \hline
\end{tabular}
\begin{flushleft} Table notes Phasellus venenatis, tortor nec vestibulum mattis, massa tortor interdum felis, nec pellentesque metus tortor nec nisl. Ut ornare mauris tellus, vel dapibus arcu suscipit sed.
\end{flushleft}
\label{table1}
\end{adjustwidth}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|cccccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Network}} &
  \multicolumn{2}{c|}{Initiation} &
  \multicolumn{3}{c|}{Cessation} &
  \multicolumn{2}{c|}{Relapse} \\ \cline{2-8} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{$\bin$} &
  \multicolumn{1}{c|}{$\bspon$} &
  \multicolumn{1}{c|}{$\gin$} &
  \multicolumn{1}{c|}{$\gspon$} &
  \multicolumn{1}{c|}{$\din$} &
  \multicolumn{1}{c|}{$\oin$} &
  $\ospon$\\ \hline
FC  & 0        & 0       & 0.011449 & 0.028117 & 0.000791 & 0.750000 & 0.118569 \\
BA  & 0.000004 & 0.00001 & 0.000004 & 0.000010 & 0.056234 & 0.013335 & 0.013335 \\
ER  & 0        & 0       & 0.005724 & 0.014059 & 0.042178 & 0        & 0.028492 \\
FHS & 0        & 0       & 0.011449 & 0.028117 & 0.028122 & 0.003334 & 0.042176 \\
LFR & 0        & 0       & 0.017173 & 0.042176 & 0.014059 & 0        & 0.056234 \\
SW  & 0        & 0       & 0        & 0        & 0.042176 & 0        & 0.014059 \\ \hline
\end{tabular}
\caption{par}
\label{tab:par}
\end{table}

